Look Around! A Neighbor Relation Graph Learning Framework for Real Estate Appraisal

Real estate appraisal is a crucial issue for urban applications, which aims to value the properties on the market. Traditional methods perform appraisal based on the domain knowledge, but suffer from the efforts of hand-crafted design. Recently, several methods have been developed to automatize the valuation process by taking the property trading transaction into account when estimating the property value. However, existing methods only consider the real estate itself, ignoring the relation between the properties. Moreover, naively aggregating the information of neighbors fails to model the relationships between the transactions. To tackle these limitations, we propose a novel Neighbor Relation Graph Learning Framework (ReGram) by incorporating the relation between target transaction and surrounding neighbors with the attention mechanism. To model the influence between communities, we integrate the environmental information and the past price of each transaction from other communities. Moreover, since the target transactions in different regions share some similarities and differences of characteristics, we introduce a dynamic adapter to model the different distributions of the target transactions based on the input-related kernel weights. Extensive experiments on the real-world dataset with various scenarios demonstrate that ReGram robustly outperforms the state-of-the-art methods. Furthermore, comprehensive ablation studies were conducted to examine the effectiveness of each component in ReGram.

==> sections/3-preliminary.tex <==
\section{Preliminaries}
\label{sec:preliminary}

In this section, we first introduce important definitions related to the real estate appraisal problem and formulate the task.

\textit{
Definition 1: \textbf{Real Estate Transaction}. Consider a set of property trading records as real estate transactions $\boldsymbol{S}$ in chronological order, a real estate transaction at the $t$-th transaction denotes $\boldsymbol{s_t}=\{s^e_t, s^o_t\} \in \boldsymbol{S}$, where $s^e_t$ is the environment feature and $s^o_t$ is the object feature.
% , $\{s^e_t, s^o_t, p_t\}$ is the environment feature, object feature and property unit price of $\boldsymbol{s_t}$ respectively.
}

\textit{
Definition 2: \textbf{Real Estate Value}. Consider a set of property unit prices as real estate value $\boldsymbol{P}$ in chronological order; a real estate value at the $t$-th transaction denotes $\boldsymbol{p_t}\in \boldsymbol{P}$, where $p_t$ is the value of the real estate transaction.
}

\textit{
Definition 3: \textbf{Target Transaction}. Target transaction $\boldsymbol{s_{t+1}}=\{s^e_{t+1}, s^o_{t+1}\}$ is the real estate transaction that will be appraised.
}

\textit{
Definition 4: \textbf{Environment Feature}. Environment features represent the surrounding environment information of the property. In this paper, we denote the PoI feature, geographic information (longitude, latitude), land usage and house age as environment features.
}

\textit{
Definition 5: \textbf{Object Feature}. Object features represent the information about the property such as the size of the house, the number of rooms in the house, and the floor number of the house, etc.
% "house size", "number of rooms", "floor number".
}

\textit{
Definition 6: \textbf{PoI Feature}. PoI (point of interest) features consist of two types of features. The first is the number of PoI with a Euclidean distance. For example, there are two schools around 5km from the property. The other is the minimum distance to each PoI category. For example, the shortest distance to the hospital or gas station.
}

\textit{
Definition 7: \textbf{Community}. A community is a hyper node containing multiple transactions that are built in the same region at the same time. In this paper, two transactions belong to the same community if and only if they meet the following conditions: (1) The completion dates (month and year) of construction are the same. (2) The distance between two transactions is less than 500m \cite{DBLP:conf/kdd/0003LZZLD021}.
}

\textit{
\textbf{Real Estate Appraisal Problem}. Given a target transaction $\boldsymbol{s_{t+1}}$ with its previous transactions $\boldsymbol{S_{[0..t]}}$ and corresponding unit price $\boldsymbol{P_{[0..t]}}$, the task is to estimate the transaction unit price $\boldsymbol{p_{t+1}}$.
}


==> tables/features_detail.tex <==
\begin{tabular}{c|c|c}
 \toprule
 Feature Type & Feature Category & Description \\
 \midrule \midrule
 \multirow{9}{*}{Transaction Feature} & Transaction Information & Number of transferred land, building number and parking space.\\
 & Property Inner Information &  Number of room, living room, bathroom, and compartment; Type of parking space.\\
 & Property Outer Information & Whether there is a management organization; Floor number; Total floor number.\\
 & Property Other Information & House age; Whether it is on the first floor; Whether it is a shop.\\
 & Geographic Location & City; Urban area; Longitude; Latitude.\\
 & Transfer Area Size &  Transfer land size, building size, parking space size, balcony size, etc.\\
 & Related Date & Trading date; Construction completed date.\\
 & Construction Detail & Construction type; Main purpose; Main building materials.\\
 & Land Information &  Category of the urban land and non-urban land.\\
 \midrule
 \multirow{2}{*}{PoI Feature} & Shortest Distance to PoI & The distance of shortest path to each PoI category.\\
 & Number of Surrounding PoI & We consider 10, 50, 100, 250, 500, 1000, 5000, 10000 meters in our work.\\
 \bottomrule
\end{tabular}


==> tables/knn_n.tex <==
\begin{tabular}{c|c}
 \toprule
  & Neighbors Number\\
 \midrule
 New Taipei & 5 \\
 Taipei & 3 \\
 Taoyuan & 4 \\
 Taichung & 9  \\
 Tainan &  8 \\
 Kaohsiung &  7 \\
 \bottomrule
\end{tabular}
